PASA: A Priori Adaptive Splitting Algorithm for the Split Delivery Vehicle Routing Problem

The split delivery vehicle routing problem (SDVRP) is a relaxed variant of the capacitated vehicle routing problem (CVRP) where the restriction that each customer is visited precisely once is removed. Compared with CVRP, the SDVRP allows a reduction in the cost of the routes traveled by vehicles. The exact methods to solve the SDVRP are computationally expensive. Moreover, the complexity and difficult implementation of the state-of-the-art heuristic approaches hinder their application in real-life scenarios of the SDVRP. In this paper, we propose an easily understandable and effective approach to solve the SDVPR based on an a priori adaptive splitting algorithm (PASA). The idea of a priori split strategy was first introduced in Chen et al. (2017). In this approach, the demand of the customers is split into smaller values using a fixed splitting rule in advance. Consequently, the original SDVRP instance is converted to a CVRP instance which is solved using an existing CVRP solver. While the proposed a priori splitting rule in Chen et al. (2017) is fixed for all customers regardless of their demand and location, we suggest an adaptive splitting rule that takes into account the distance of the customers to the depot and their demand values. Our experiments show that PASA can generate solutions comparable to the state-of-the-art but much faster. Furthermore, our algorithm outperforms the fixed a priori splitting rule proposed by Chen et al. (2017).

==> results+ILS-MIP.tex <==

% \begin{landscape}
% \begin{table}[t]
%     \centering
%     \caption{Performance of RSR on Set-1}
% \begin{tabular}{ccccccccccc}
%  \hline
%  Instance & Best-known &  \multicolumn{3}{c}{VRPHAS (Our runs)} &  \multicolumn{3}{c}{RSR}  &  \multicolumn{2}{c}{No Splitting}\\
%   & & cost & gap ($\%$) & time (s) & cost & gap ($\%$) & time (s) & cost & gap ($\%$)\\
%  \hline
%   SD1 & 228.28 & 228.28 (228.28) & 0.00 (0.00) & 0.59 (0.51) & 228.28  & 0.00  & 1.60 & 240 & 5.13 \\
%   SD2 & 708.28 & 708.28 (708.280 & 0.00 (0.00) & 1.65 (1.23) & 708.28  & 0.00  & 2.85 & 800 & 12.94 \\
%   SD3 & 430.40 & 430.58 (430.58) & 0.04 (0.04) & 1.62 (1.25) & 430.58  & 0.04  & 2.57 & 479.97 & 11.51\\
%   SD4 & 630.62 & 631.05 (631.05) & 0.07 (0.07) & 3.01 (2.35) & 631.04  & 0.07  & 3.57 & 719.99 & 14.17\\
%   SD5 & 1389.94 & 1390.57 (1406.90) & 0.05 (1.22) & 4.59 (3.91) & 1390.57  & 0.05 & 5.66 & 1599.95 & 15.10\\
%   SD6 & 830.86 & 831.24 (831.24) & 0.05 (0.05) & 4.04 (3.85) & 831.24 & 0.05 & 5.09 & 960 & 15.47\\
%   SD7 & 3640.00 & 3640.00 (3660.00) & 0.00 (0.55) & 9.22 (5.47) & 3640.00 & 0.00 & 7.79 & 4400 & 20.87\\
%   SD8 & 5068.28 & 5068.28 (5068.28) & 0.00 (0.00) & 14.51 (7.64) & 5068.28 &  0.00 & 10.43  & 6240 & 23.11\\
%   SD9 & 2042.88 & 2057.62 (2057.62) & 0.72 (0.72) & 7.34 (7.5) & 2051.06 & 0.40 & 8.97 & 2399.96 & 17.47 \\
%   SD10 & 2683.73 & 2707.83 (2709.26) & 0.90 (0.95) & 16.87 (13.73) & 2704.88 & 0.79 & 13.68 & 3200.04 & 19.23\\
%   SD11 & 13280.00 & 13280.00 (13300.00) & 0.00 (0.15) & 25.14 (20.59) & 13480.00 & 1.50 & 18.43 & 16800 & 26.50  \\
%   SD12 & 7213.62 & 7259.46 (7266.48) & 0.64 (0.73) & 24.08 (20.89) & 7238.88 & 0.34 & 20.99 & 8799.96 & 21.99\\
%   SD13 & 10105.86 & 10110.58 (10110.58) & 0.05 (0.05) & 27.14 (25.90) & 10110.58 & 0.05 & 22.05 & 12479.95 & 23.49\\
%   SD14 & 10717.53 & 10771.54 (10792.22) & 0.51 (0.70) & 33.54 (42.57) & 10804.84 & 0.81 & 32.03 & 13200 & 23.16\\
%   SD15 & 15094.48 & 15250.13 (15235.32) & 1.03 (0.93) & 41.46 (59.43) & 15232.60 & 0.91 & 47.32 & 18720 & 24.01\\
%   SD16 & 3379.33 & 3553.32 (3565.44) & 5.15 (5.50) & 17.95 (54.88) & 3508.16 & 3.81 & 30.16 & 4319.94 & 27.83\\
%   SD17 & 26493.56 & 26547.06 (26559.40) & 0.20 (0.25) & 51.29 (66.98) & 26962.64 & 1.56 & 50.14 & 33599.91 & 26.82\\
%   SD18 & 14202.53 & 14320.66 (14301.00) & 0.83 (0.69) & 50.08 (72.04) & 14278.70 & 0.54 & 54.75 & 17600.01 & 23.92\\
%   SD19 & 19995.69 & 20251.89 (20196.51) & 1.28 (1.00) & 52.80 (101.05) & 20197.04 & 1.00 & 70.14 & 24960.01 & 24.82\\
%   SD20 & 39635.51 & 39678.10 (39701.85) & 0.11 (0.17) & 80.94 (162.9) & 40236.66 & 1.51 & 104.51 & 50399.98 & 27.15\\
%   SD21 & 11271.06 & 11631.67 (11656.37) & 3.20 (3.41) & 105.20 (240.36) & 11576.96 & 2.71 & 129.31 & 14400 & 27.76 \\
%   \hline
%   Average & & & 0.71 (0.82) & 27.29 (86.14) & & 0.76 & 30.56 & & 20.60\\
%  \hline
% \end{tabular}
% \end{table}
% \end{landscape}

% \begin{landscape}
\begin{table}[t]
    \centering
    \caption{Performance of RSR on Set-1}
\begin{tabular}{ccccccccccc}
 \hline
 Instance & Best-known &  \multicolumn{2}{c}{VRPHAS (Our runs)} &  \multicolumn{3}{c}{RSR}  & \multicolumn{2}{c}{{ILS-MIP}}  &\multicolumn{1}{c}{No Splitting}\\
  & & gap ($\%$) & time (s) & cost & gap ($\%$) & time (s) &gap  & time(s) & gap ($\%$) \\
 \hline
  SD1 & 228.28  & 0.00 & 0.51 & 228.28  & 0.00  & 1.60  &\red{0.00} & \red{25.10} - \blue{0.00} & 5.13 \\
  
  SD2 & 708.28 & 0.00 & 1.23 & 708.28 & 0.00 & 2.85  &\red{0.00} & \red{47.51} - \blue{0.00} & 12.94 \\
  
  SD3 & 430.40   & 0.04 & 1.25 & 430.58  & 0.04  & 2.57 &\red{0.05}& \red{37.68} - \blue{0.00} & 11.51\\
  
  SD4 & 630.62  & 0.07 &  2.35 & 631.04  & 0.07  & 3.57 &\red{0.07} & \red{75.45} - \blue{0.00} & 14.17\\
  
  SD5 & 1389.94  & 1.22 & 3.91 & 1390.57  & 0.05  & 5.66 &\red{0.05}& \red{216.69} - \blue{0.80} & 15.10\\
  
  SD6 & 830.86  & 0.05 & 3.85 & 831.24 & 0.05  & 5.09 &\red{0.04}& \red{202.60} - \blue{92.42} & 15.47\\
  
  SD7 & 3640.00  & 0.55 & 5.47 & 3640.00 & 0.00  & 7.79  &\red{0.00}& \red{tl} - \blue{0.00} & 20.87\\
  
  SD8 & 5068.28  & 0.00 & 7.64 & 5068.28 & 0.00 & 10.43  &\red{0.00}& \red{tl} - \blue{0.00} & 23.11\\
  
  SD9 & 2042.88  & 0.72 & 7.50 & 2051.06 & 0.40  & 8.97  &\red{0.07} & \red{tl} - \blue{39187} & 17.47 \\
  
  SD10 & 2683.73 & 0.95 & 13.73 & 2704.88 & 0.79  & 13.68   &\red{0.38} & \red{tl} - \blue{960.42} & 19.23\\
  
  SD11 & 13280.00  & 0.15 &20.59 & 13480.00 & 1.50  & 18.43   &\red{0.00} & \red{tl} - \blue{0.00} & 26.50  \\
  
  SD12 & 7213.62  &  0.73 & 20.89 & 7238.88 & 0.34  & 20.99   &\red{0.09} & \red{tl} - \blue{1223.31} & 21.99\\
  
  SD13 & 10105.86  & 0.05 & 25.90 & 10110.58 & 0.05  & 22.05   &\red{0.05} & \red{tl} - \blue{1091.84} & 23.49\\
  
  SD14 & 10717.53 & 0.70 & 42.57 & 10804.84 & 0.81  & 32.03   &\red{0.22} & \red{tl} - \blue{967.30} & 23.16\\
  
  SD15 & 15094.48  & 0.93 & 59.43 & 15232.60 & 0.91  & 47.32  &\red{0.37} & \red{tl} - \blue{318.44} & 24.01\\
  
  SD16 & 3379.33  & 5.50 & 54.88 & 3508.16 & 3.81  & 30.16   &\red{0.11} & \red{tl} - \blue{0.01} & 27.83\\
  
  SD17 & 26493.56  & 0.25 & 66.98 & 26962.64 & 1.56  & 50.14   &\red{ 0.1} & \red{tl} - \blue{1328.05} & 26.82\\
  
  SD18 & 14202.53  &0.69 &72.04 & 14278.70 & 0.54 & 54.75   &\red{0.46}& \red{tl} - \blue{1347.05} & 23.92\\
  
  SD19 & 19995.69  & 1.00 & 101.05 & 20197.04 & 1.00  & 70.14   &\red{0.64} & \red{tl} - \blue{1328.17} & 24.82\\
  
  SD20 & 39635.51  &0.17 & 162.90 & 40236.66 & 1.51 & 104.51   &\red{0.25} & \red{tl} - \blue{1328.44} & 27.15\\
  
  SD21 & 11271.06  & 3.41 &240.36 & 11576.96 & 2.71  & 129.31  &\red{0.2} & \red{tl} - \blue{0.00} & 27.76 \\
  \hline
  Average & & 0.82 & 86.14 & & 0.76 & 30.56  & \red{0.15} &\red{tl!} - \blue{494.17} & 20.60\\
 \hline
\end{tabular}
\end{table}
% \end{landscape}

% \begin{landscape}
% \begin{table}[t]
% \centering
% \caption{Performance of RSR on SET-2}
% \begin{tabular}{cccccccccc}
%  \hline
%  Instance & Best-known &  \multicolumn{3}{c}{VRPHAS (Our runs)} &  \multicolumn{3}{c}{RSR} &  \multicolumn{2}{c}{No Splitting}  \\
%   & & cost & gap ($\%$) & time (s) & cost & gap ($\%$) & time (s)  & cost & gap ($\%$) \\
%  \hline
% S51D1 & 459.50  & 459.50 (459.50) & 0.00 (0.00) & 7.23 (10.98) & 459.50 & 0.00 & 7.92 & 459.5 & 0.00 \\ 
% S51D2 &  709.29 & 716.82 (714.79) & 1.06 (0.77) & 11.46 (15.04) & 713.80  & 0.63  & 11.22 & 721.47 & 1.71 \\ 
% S51D3 & 948.06 & 964.83 (965.86)  & 1.77 (1.88)  & 15.88 (20.28)  & 959.92  & 1.25 & 13.04 & 978.33 & 3.19 \\ 
% S51D4 & 1562.01 & 1592.23 (1592.35) & 1.93 (1.94) & 18.90 (28.24) & 1583.88 & 1.40 & 22.94 & 1676.41 & 7.32 \\
% S51D5 & 1333.67 &  1371.41 (1347.44) & 2.83 (1.03)  & 19.66 (30.68)  & 1343.109  & 0.71  & 20.81 & 1452.28 & 8.89\\ 
% S51D6 & 2169.10 & 2240.46 (2209.40)  & 3.29 (1.86) &  28.04 (43.81)&  2211.90  & 1.97 & 23.37 & 2402.34 & 10.75\\ 
% S76D1 & 598.94 &  614.31 (598.94) &  2.57 (0.00) & 15.07 (23.18)  & 598.94 & 0.0 & 14.55 & 603.63 & 0.78 \\ 
% S76D2 & 1087.40 & 1120.71 (1107.22)  & 3.06 (1.82)  & 21.54 (32.48)  & 1104.88 & 1.61 & 22.43 & 117.77 & 2.79 \\ 
% S76D3 & 1427.86 & 1445.23 (1455.39) & 1.22 (1.93) & 34.28 (46.99) & 1436.99 & 0.64 & 28.05 & 1463.85 & 2.52 \\ 
% S76D4 &  2079.76  & 2138.64 (2131.91)  & 2.83 (2.51) & 29.74 (55.89)  & 2120.16 & 1.94 & 40.09 & 2192.37 & 5.41\\ 
% S101D1 & 726.59 & 746.08 (735.51) &  2.68 (1.23) & 22.02 (34.03) & 729.72 & 0.43 & 42.31 & 734.94 & 1.14\\ 
% S101D2 & 1378.43 & 1412.98 (1406.08)  & 2.51 (2.00)  &  37.16 (52.44) & 1399.67 & 1.54 & 34.45 & 1401.56 & 1.67 \\ 
% S101D3 &  1874.81 & 1924.39 (1909.52) & 2.64 (1.85) & 39.49 (70.64) &  1905.43 & 1.63 & 41.05 & 1952.27 & 4.13\\ 
% S101D5 & 2791.22 & 2874.86 (2836.26) & 3.00 (1.61) & 45.44 (95.71) & 2844.51 & 1.91 & 62.54 & 3114.84 & 11.59
% \\\hline
% Average &   & & 2.24 (1.45) & 24.71 (40.02) &  & 1.13 & 28.18  & & 4.42\\
% \hline
% \end{tabular}
% \end{table}
% \end{landscape}
% \begin{landscape}
\begin{table}[t]
    \centering
    \caption{Performance of RSR on Set-2}
\begin{tabular}{ccccccccccc}
 \hline
 Instance & Best-known &  \multicolumn{2}{c}{VRPHAS (Our runs)} &  \multicolumn{3}{c}{RSR}  & \multicolumn{2}{c}{{ILS-MIP}}  &\multicolumn{1}{c}{No Splitting}\\
  & & gap ($\%$) & time (s) & cost & gap ($\%$) & time (s) &gap($\%$)  & time(s) & gap ($\%$) \\
 \hline
S51D1 & \red{458.00}  & 0.32 & 10.98 & 459.5 & 0.32 & 7.92 & \red{0.00} & \red{160.36} - \blue{0.16}  & 0.32 \\ 

S51D2 & \red{703.00} & 1.68 & 15.04 & 713.80  & 1.49  & 11.22 & \red{0.00} & \red{tl} - \blue{1020.02}  & 2.63 \\ 

S51D3 & \red{945.00} & 2.21  & 20.28  & 959.92  & 1.58 & 13.04 & \red{0.00} & \red{tl} - \blue{12.12}  & 3.53 \\ 

S51D4 & \red{1553.00}  & 2.53 & 28.24 & 1583.88 & 1.99 & 22.94 & \red{0.00} & \red{tl} - \blue{1225.99}  & 7.95 \\

S51D5 & \red{1328.00}  & 1.46  & 30.68  & 1343.11  & 1.13& 20.81 & \red{0.00} & \red{tl} - \blue{183.70}  & 9.36\\ 

S51D6 & \red{2166.00}   & 1.99 &  43.81&  2211.90  & 2.12& 23.37 & \red{0.00} & \red{tl} - \blue{129.67}  & 10.91\\ 

S76D1 &\red{592.00}  &  1.17 & 23.18 & 598.94 & 1.17 & 14.55 & \red{0.00}& \red{626.75} - \blue{87.06}  & 1.96 \\ 

S76D2 &  \red{1082.00}  & 2.33  & 32.48  & 1104.88 & 2.03 & 22.43 & \red{0.00} & \red{tl} - \blue{55.97} & 3.30 \\ 

S76D3 &  \red{1422.00}  & 2.35 & 46.99 & 1436.99 & 1.05 & 28.05 & \red{0.00} & \red{tl} - \blue{1133.87}  & 2.94 \\ 

S76D4 &  \red{2078.00}   & 2.59 & 55.89 & 2120.16 & 2.03 & 40.09 & \red{0.00}& \red{tl} - \blue{979.46}  & 5.50\\ 

S101D1 & \red{716.00}  &  2.72 & 34.03 & 729.72 & 1.91& 42.31 & \red{0.00}  & \red{tl} - \blue{34.99}& 2.65\\ 

S101D2 & \red{1368.00}   & 2.78  &  52.44 & 1399.67 & 2.32  & 34.45& \red{0.00} & \red{tl} - \blue{424.75}  & 2.45 \\ 

S101D3 & \red{1869.00}  & 2.17 & 70.64 &  1905.43 & 1.95 & 41.05 & \red{0.00} & \red{tl} - \blue{216.97}  & 4.46\\ 

S101D5 & \red{2778.00} & 2.09 & 95.71 & 2844.51 & 2.39 & 62.54  & \red{0.00} & \red{tl} - \blue{965.43} & 12.12
\\\hline
Average &  & 2.02 & 40.02 &  & 1.67 & 28.18 & 0.00 & \red{tl!} - \blue{462.15}  & 5.00\\
\hline
\end{tabular}
\end{table}
% \end{landscape}


{\small
% \begin{landscape}
\begin{table}[t]
    \centering
    \caption{Performance of RSR on SET-3}
\begin{tabular}{ccccccccccc}
 \hline
 Instance & Best-known &  \multicolumn{2}{c}{VRPHAS (Our runs)} &  \multicolumn{3}{c}{RSR}  & \multicolumn{2}{c}{{ILS-MIP}}  &\multicolumn{1}{c}{No Splitting}\\
  & & gap ($\%$) & time (s) & cost & gap ($\%$) & time (s) &gap  & time(s) & gap ($\%$) \\
 \hline
p01\_110  & 458.00  & 0.33 & 9.84 & 459.50  & 0.00  & 6.63 & 0.00 & 160.10 - 0.04 & 0.33\\ 

p01\_1030 & 753.00 & 1.74 & 17.2 & 770.93 & 2.38 & 11.0 & 0.00 & tl - 339.32 & 3.86\\


p01\_1050 & 998.00  & 3.35 & 22.52 & 1021.18 & 2.32 & 15.76 & 0.00 & tl - 290.2& 4.90\\ 


p01\_1090 & 1481.00 & 2.00 & 32.70 & 1507.14 & 1.77  & 19.61 & 0.00 & tl - 642.66 & 13.34\\ 

p01\_3070 & 1474.00  & 2.71 & 32.84 & 1503.66 & 2.01 & 17.02 & 0.00 & tl - 596.27  & 14.41\\ 

p01\_7090 & 2151.00 & 2.49 & 49.82 & 2203.93 & 2.46 & 21.41 & 0.00 & tl - 562.15 & 11.69\\ 

p02\_110 &  612.00 & 1.62 & 21.82 & 618.13 & 1.00 & 12.08 & 0.00 & tl - 63.96 & 1.62\\


p02\_1030 & 1109.00  & 1.70 & 28.86 & 1125.65 & 1.50 & 21.83  & 0.00 & tl - 959.81 & 2.57\\ 

p02\_1050 & 1497.00 & 1.40 & 22.52 & 1508.98 & 0.80 & 26.21 & 0.00 & tl - 1249.87 & 3.07\\ 

p02\_1090 & 2291.00 & 2.33 & 61.01 & 2334.33 & 1.89 & 41.19 & 0.00 & tl - 1255.71 & 9.57\\ 

p02\_3070 & 2219.97 & 2.23 & 58.80 &  2269.50 & 2.23 & 28.02 & 0.05 & tl - 1215.81 & 12.87\\ 


p02\_7090 & 3220.00  & 1.67 & 89.76 & 3305.53 & 2.66 & 40.52 & 0.00 & tl - 1323.51 & 12.76\\ 


p03\_110 &  749.00 & 2.26 & 55.12 & 762.54  & 1.80 & 22.08 & 0.00 & tl - 70.94 & 2.00\\ 


p03\_1030 & 1453.00  & 2.26 & 37.26 & 1476.86 & 1.64 & 35.67  & 0.00 & tl - 786.74 & 2.48\\ 


p03\_1050 & 1996.76 & 1.06 & 58.40 & 2032.25 & 1.77 & 41.76 & 0.01 & tl - 837.40 & 3.93\\ 


p03\_1090 & 3085.69 & 2.29 & 143.32 &  3143.69 & 1.88 & 56.56 & 0.04 & tl - 682.60 & 12.17\\ 

p03\_3070 & 2985.00  & 2.34 & 136.10 & 3034.28 & 1.65 & 40.02 & 0.00 & tl - 1315.41 & 16.67\\ 

p03\_7090 & 4374.00 & 1.97 & 186.14 & 4464.65 & 2.07 & 84.48 & 0.00 & 1282.20 & 14.06\\ 
% \hline
% \end{tabular}
% \end{table}
% % \end{landscape}

% % \begin{landscape}
% \begin{table}[t]
%     \centering
%     \caption{Continued}
% \begin{tabular}{ccccccccccc}
%  \hline
%  Instance & Best-known &  \multicolumn{2}{c}{VRPHAS (Our runs)} &  \multicolumn{3}{c}{RSR}  & \multicolumn{2}{c}{{ILS-MIP}}  &\multicolumn{1}{c}{No Splitting}\\
%   & & gap ($\%$) & time (s) & cost & gap ($\%$) & time (s) &gap  & time(s) & gap ($\%$) \\
%  \hline
p04\_110 & 910.00  & 2.38 & 116.08 & 925.19  & 1.67 & 33.83 & 0.00 & tl- 164.85 & 1.86 \\ 

p04\_1030 & 2012.00 & 2.96 & 152.44 &  2056.71 & 2.22 & 55.37 & 0.00 & tl - 428.34 & 3.22\\ 

p04\_1050 & 2849.66  & 2.40 & 196.82 & 2889.62 & 1.40 & 72.14  & 0.40 & tl - 893.97 & 5.09\\ 

p04\_1090 & 4545.46 &  2.44 & 310.84 & 4624.18 & 1.73 & 112.41 & 0.21 & tl - 1328.07 & 14.72\\

p04\_3070 & 4334.71  & 2.87 & 272.44 & 4407.02 & 1.67 & 99.65 & 0.65 & tl - 1328.10 & 19.64\\ 

p04\_7090 & 6395.41 & 1.94 & 469.62 & 6555.47 & 2.5 & 82.07 & 0.90 & tl - 1227.11 & 15.09\\ 

p05\_110 &  1059.00  & 4.22 & 186.66 & 1086.27 & 2.58 & 66.5 & 0.00 & tl - 834.72 & 2.88 \\ 

p05\_1030 & 2478.40 & 1.83 & 241.44 & 2515.45 & 1.49 & 82.72 & 0.51 & tl - 721.58 & 2.46\\ 

p05\_1050 & 3471.41 & 1.54 & 311.94 & 3510.99 & 1.14 & 87.56 & 0.77 & tl - 1328.24 & 4.01\\

p05\_1090 & 5521.57 & 2.02 &  561.54 & 5619.52 & 1.77 & 145.02 & 2.12 & tl - 1053.99 & 12.67\\ 

p05\_3070 & 5409.76  & 2.41 & 383.28 & 5412.85 & 0.06 & 142.81 & 1.65 & tl - 1328.12  & 15.57\\ 

p05\_7090 & 8192.03 & 1.96 & 884.68 & 8332.36 & 1.71 & 255.05 & 0.38 & tl - 1328.14 & 17.28\\

p11\_110 & 1030.00 & 2.22 & 74.12 & 1044.44 & 1.36  & 20.20 & 0.00 & tl - 934.18 & 1.67\\

p11\_1030 & 2881.80 & 2.89 & 94.06 &  2923.86 & 1.46  & 40.64 & 0.42 & tl - 1230.56 & 1.95\\ 

p11\_1050 & 4219.01  & 2.29 & 108.54 & 4268.79 & 1.18 & 55.27 & 0.05 & tl - 815.47 & 2.71\\

p11\_1090 & 6854.09  & 3.27 & 188.30 &  6994.56 & 2.05 & 64.06 & 0.16 & tl - 1135.73 & 13.22\\ 

p11\_3070 & 6646.00  & 1.82 & 162.36 & 6759.99 & 1.72 & 59.01 & 0.00 & tl - 1346.85 & 16.24\\

p11\_7090 & 10204.81  & 1.99 & 231.60 & 10406.25 & 1.97 & 101.02 & 0.13 & tl - 1328.08 & 19.93\\ \hline
Average &  & & 1.50 (1.96) & 45.51 (166.94) & & 1.45 & 33.38 & & 8.08 \\\hline
\end{tabular}
\end{table}
% \end{landscape}
}
% \begin{table}[H]
% %\label{table:equil}
% \centering
% \caption{Performance of RSR on SET-3}
% \begin{tabular}{cccc}
% \hline
% Instance  &  Best Known &  \multicolumn{2}{c}{No splitting}  \\\hline
%   & & cost & gap($\%$) \\
%  \hline
% p01\_110  & 459.50 &  459.50 & 0.00\\ 
% p01\_1030 & 757.17 & 782.097 & 3.29\\ 
% p01\_1050 & 1005.75   &  1046.88 & 4.08\\ 
% p01\_1090 & 1488.58   &  1678.51 & 12.75\\ 
% p01\_3070 & 1481.71   &  1686.37 & 13.81\\ 
% p01\_7090 & 2156.14   &  2402.35 & 11.41\\  
% p02\_110 &  617.85  &  621.92 & 0.65\\ 
% p02\_1030 & 1109.62   &  1137.47 & 2.50\\ 
% p02\_1050 & 1502.05   &  1542.97 & 2.72\\ 
% p02\_1090 & 2298.58   &  2510.34 & 9.21\\ 
% p02\_3070 & 2219.97   &  2505.86 & 12.87\\ 
% p02\_7090 & 3223.4   &  3630.86 & 12.64\\ 
% %p03\_00 &    &   &   &   &   &   & \\\hline
% p03\_110 &  752.62  &  763.99 & 1.51\\ 
% p03\_1030 & 1458.46   &  1489.08 & 2.09\\ 
% p03\_1050 & 1996.76   &  2075.26 & 3.93\\ 
% p03\_1090 & 3085.69   &  3461.54 & 12.17\\ 
% p03\_3070 & 2989.3   &  3482.66 & 16.50\\ 
% p03\_7090 & 4387.32   & 4989.42  & 13.72\\ 
% %p04\_00 &    &   &   &   &   &   & \\\hline
% p04\_110 &  919.17  & 926.91  & 0.84\\ 
% p04\_1030 & 2016.97   & 2076.88 & 2.97\\ 
% p04\_1050 & 2849.66   &  2994.89 & 5.09\\ 
% p04\_1090 & 4545.46   &  5214.80 & 14.72\\ 
% p04\_3070 & 4334.71   & 5186.12 & 19.64\\ 
% p04\_7090 & 6395.41   &  7360.50 & 15.09\\ 
% %p05\_00 &    &   &   &   &   &   & \\\hline
% p05\_110 &  1074.18  &  1089.50 & 1.42\\ 
% p05\_1030 & 2478.4   &  2539.43 & 2.46\\ 
% p05\_1050 & 3471.41   & 3610.86 & 4.01\\ 
% p05\_1090 & 5521.57   &  6221.60 & 12.67\\ 
% p05\_3070 & 5409.76   &  6252.18  & 15.57\\ 
% p05\_7090 & 8192.03   & 9608.41 & 17.28\\ 
% %p11\_00 &    &   &   &   &   &   & \\\hline
% p11\_110 & 1031.11   & 1047.17 & 1.55\\ 
% p11\_1030 & 2881.8   &  2938.20 & 1.95\\ 
% p11\_1050 & 4219.01   &  4333.50 & 2.71\\
% p11\_1090 & 6854.09   &  7760.30 & 13.22\\ 
% p11\_3070 & 6671.04   & 7725.04 & 15.79\\ 
% p11\_7090 & 10204.81   & 12239.31 & 19.93\\ \hline
% Average &     &   & 8.08\\ \hline
% \end{tabular}
% %\end{center}
% \end{table}


% \begin{landscape}
\begin{table}[t]
\centering
\caption{Performance of RSR on Set-4}
\begin{tabular}{ccccccccccc}
 \hline
 Instance & Best-known &  \multicolumn{2}{c}{VRPHAS (Our runs)} &  \multicolumn{3}{c}{RSR}  & \multicolumn{2}{c}{{ILS-MIP}}  &\multicolumn{1}{c}{No Splitting}\\
  & & gap ($\%$) & time (s) & cost & gap ($\%$) & time (s) &gap  & time(s) & gap ($\%$) \\
 \hline
 eil22 & 375.28  & 0.00 & 3.28 & 375.28 & 0.00 & 3.11 & 0.00 & 49.53 - 0.00 & 0.00\\
 
 eil23 & 568.56 & 0.00 & 5.92 & 568.56 & 0.00 & 2.92 & 0.00 & 44.72 - 0.00 & 0.00 \\
 
 eil30 & 497.53 & 1.50 & 6.89 & 505.01 & 1.50 & 3.64 & 1.9 & 63.72 - 0.00 & 1.48 \\
 
 eil33 & 826.41 & 1.36 & 6.89 & 837.67 & 1.36 & 5.08 & 1.03 & 74.50 - 0.01 & 1.36\\
 
 eil51 & 521.00 & 0.69 & 12.58 & 524.61 & 0.69 & 10.95 & 199.27 & 0.08 & 0.69\\
 
 eilA76 &  823.89 & 849.60 (827.47) & 3.12 (0.43)  & 17.76 (24.60) & 830.97 & 0.86 & 19.77 & 837.45 & 1.61\\
 
 eilB76 & 1009.04  & 1024.44 (1028.80)  & 1.53 (1.96) & 18.81 (31.86) & 1025.24 & 1.60 & 18.65 & 1028.23 & 1.86\\
 eilC76 &  738.67 & 748.51 (742.81) &  1.33 (0.52) & 15.36 (26.78) & 742.49 & 0.55 & 17.48 & 743.48 & 0.64\\
 eilD76 & 684.53 & 684.53 (690.09) & 0.00 (0.81) & 14.72 (23.82) & 689.47 & 0.72 & 19.41  & 690.20 & 0.82\\
 eilA101 & 812.51 & 812.51 (831.65) & 0.00 (2.35) & 14.73 (55.39) & 828.98 & 2.02 & 23.37 & 827.39 & 1.92\\
 eilB101 &  1076.26  &  1099.21 (1093.13) & 2.13 (1.57) & 21.61 (30.90) & 1087.70 & 1.06 & 23.76 & 1093.02 & 1.53\\
 \hline
 Average & & & 0.74 (0.96) & 11.03 (20.80) & & 0.88 & 13.63 &  & 1.02\\
 \hline
\end{tabular}
\end{table}
% \end{landscape}

==> resultsSet2-4.tex <==
\begin{landscape}
\begin{table}[t]
\caption{Performance of RSR on SET-2}
\centering
\begin{tabular}{cccccccccc}
 \hline
 Instance & Best-known &  \multicolumn{3}{c}{VRPHAS (Our runs)} &  \multicolumn{3}{c}{RSR} &  \multicolumn{2}{c}{No Splitting}  \\
  & & cost & gap ($\%$) & time (s) & cost & gap ($\%$) & time (s)  & cost & gap ($\%$) \\
 \hline
S51D1 & 459.50  & 459.50 (459.50) & 0.00 (0.00) & 7.23 (10.98) & 459.50 & 0.00 & 7.92 & 459.5 & 0.00 \\ 
S51D2 &  709.29 & 716.82 (714.79) & 1.06 (0.77) & 11.46 (15.04) & 713.80  & 0.63  & 11.22 & 721.47 & 1.71 \\ 
S51D3 & 948.06 & 964.83 (965.86)  & 1.77 (1.88)  & 15.88 (20.28)  & 959.92  & 1.25 & 13.04 & 978.33 & 3.19 \\ 
S51D4 & 1562.01 & 1592.23 (1592.35) & 1.93 (1.94) & 18.90 (28.24) & 1583.88 & 1.40 & 22.94 & 1676.41 & 7.32 \\
S51D5 & 1333.67 &  1371.41 (1347.44) & 2.83 (1.03)  & 19.66 (30.68)  & 1343.109  & 0.71  & 20.81 & 1452.28 & 8.89\\ 
S51D6 & 2169.10 & 2240.46 (2209.40)  & 3.29 (1.86) &  28.04 (43.81)&  2211.90  & 1.97 & 23.37 & 2402.34 & 10.75\\ 
S76D1 & 598.94 &  614.31 (598.94) &  2.57 (0.00) & 15.07 (23.18)  & 598.94 & 0.0 & 14.55 & 603.63 & 0.78 \\ 
S76D2 & 1087.40 & 1120.71 (1107.22)  & 3.06 (1.82)  & 21.54 (32.48)  & 1104.88 & 1.61 & 22.43 & 117.77 & 2.79 \\ 
S76D3 & 1427.86 & 1445.23 (1455.39) & 1.22 (1.93) & 34.28 (46.99) & 1436.99 & 0.64 & 28.05 & 1463.85 & 2.52 \\ 
S76D4 &  2079.76  & 2138.64 (2131.91)  & 2.83 (2.51) & 29.74 (55.89)  & 2120.16 & 1.94 & 40.09 & 2192.37 & 5.41\\ 
S101D1 & 726.59 & 746.08 (735.51) &  2.68 (1.23) & 22.02 (34.03) & 729.72 & 0.43 & 42.31 & 734.94 & 1.14\\ 
S101D2 & 1378.43 & 1412.98 (1406.08)  & 2.51 (2.00)  &  37.16 (52.44) & 1399.67 & 1.54 & 34.45 & 1401.56 & 1.67 \\ 
S101D3 &  1874.81 & 1924.39 (1909.52) & 2.64 (1.85) & 39.49 (70.64) &  1905.43 & 1.63 & 41.05 & 1952.27 & 4.13\\ 
S101D5 & 2791.22 & 2874.86 (2836.26) & 3.00 (1.61) & 45.44 (95.71) & 2844.51 & 1.91 & 62.54 & 3114.84 & 11.59
\\\hline
Average &   & & 2.24 (1.45) & 24.71 (40.02) &  & 1.13 & 28.18  & & 4.42\\
\hline
\end{tabular}
\end{table}
\end{landscape}


\begin{landscape}
\begin{table}[t]
 \caption{Performance of RSR on SET-3}
    \centering
\begin{tabular}{cccccccccccccccc}
 \hline
 Instance & Best-known &  \multicolumn{3}{c}{VRPHAS (Our runs)} &  \multicolumn{3}{c}{RSR} &  \multicolumn{2}{c}{No splitting} \\
  & & cost & gap ($\%$) & time (s) & cost & gap ($\%$) & time (s) & cost & gap ($\%$)\\
 \hline
p01\_110  & 459.50  & 459.50 (459.5) & 0.00(0.0) & 6.55 (9.84) & 459.50  & 0.00  & 6.63 & 459.50 & 0.00\\ 
p01\_1030 & 757.17 & 776.06 (770.35) & 2.50 (1.74) & 15.54 (17.2) & 770.93 & 1.81 & 11.08 & 782.097 & 3.29\\
p01\_1050 & 1005.75 & 1027.92 (1031.48)  & 2.21 (2.56) & 15.87 (22.52) &  1021.18 & 1.53 &  15.76 & 1046.88 & 4.08\\ 
p01\_1090 & 1488.58 & 1525.09 (1510.62) & 2.45 (1.48) & 22.07 (32.70)  & 1507.14  & 1.24  & 19.61 &  1678.51 & 12.75\\ 
p01\_3070 & 1481.71 & 1511.66 (1514.71)  & 2.02 (2.23) & 22.47 (32.84) & 1503.66 & 1.48 & 17.02 &  1686.37 & 13.81\\ 
p01\_7090 & 2156.14 & 2215.09 (2204.51)  & 2.73 (2.24) & 26.32 (49.82) & 2203.93 &  2.22 & 21.41  &  2402.35 & 11.41\\ 
p02\_110 &  617.85  & 628.86 (621.92) & 1.79 (0.66) & 10.83 (21.82) & 618.13 & 0.04 &12.08  &  621.92 & 0.65\\
p02\_1030 & 1109.62   & 1137.43 (1127.89) & 2.50 (1.65) & 23.08 (28.86) & 1125.65 & 1.44 & 21.83  &  1137.47 & 2.50\\ 
p02\_1050 & 1502.05   & 1520.83 (1517.98) & 1.25 (1.06) & 28.19 (22.52) & 1508.98  & 0.46 & 26.21&  1542.97 & 2.72\\ 
p02\_1090 & 2298.58   & 2356.70 (2344.48) & 2.53 (2.00) & 32.42 (61.01) & 2334.33 & 1.55 & 41.19  &  2510.34 & 9.21\\ 
p02\_3070 & 2219.97  & 2286.06 (2269.57) & 2.97 (2.23) & 43.51 (58.80) &  2269.50 & 2.23 & 28.02 &  2505.86 & 12.87\\ 
p02\_7090 & 3223.4   & 3303.98 (3273.89) & 2.50 (1.57) & 44.78 (89.76) & 3305.53 & 2.54 & 40.52 &  3630.86 & 12.64\\ 
p03\_110 &  752.62  & 752.62 (765.99) & 0.00 (1.78) & 13.76 (55.12) & 762.54  & 1.31 & 22.08 &  763.99 & 1.51\\ 
p03\_1030 & 1458.46   & 1469.84 (1485.82) & 0.78 (1.87) & 22.70 (37.26) &  1476.86 & 1.26 & 35.67  &  1489.08 & 2.09\\ 
p03\_1050 & 1996.76 & 2017.94 (2047.42) & 1.06 (1.06) & 29.37 (58.40) & 2032.25 & 1.77 & 41.76  &  2075.26 & 3.93\\ 
p03\_1090 & 3085.69   & 3143.09 (3156.24) & 1.86 (2.29) & 40.35 (143.32) &  3143.69 & 1.88 & 56.56  &    3461.54 & 12.17\\ 
p03\_3070 & 2989.3   & 3044.73 (3054.83) & 1.85 (2.19) & 40.98 (136.10) & 3034.28 & 1.50 & 40.02   &  3482.66 & 16.50\\ 
p03\_7090 & 4387.32  & 4475.32 (4460.09) & 2.01 (1.66) & 52.49 (186.14) & 4464.65 & 1.76 & 84.48  & 4989.42  & 13.72\\ 
p04\_110 &  919.17  &  919.17 (931.62) &  0.00 (1.35) &  30.30 (116.08) & 925.19  & 0.65 & 33.83 & 926.91  & 0.84 \\ 
p04\_1030 & 2016.97  &  2039.21 (2071.58) & 1.10 (2.71) &  40.70 (152.44)&  2056.71 & 1.97 & 55.37 & 2076.88 & 2.97\\ 
p04\_1050 & 2849.66  & 2876.70 (2918.1) & 0.95 (2.40) & 58.02 (196.82)  & 2889.62 &  1.40 & 72.14   &  2994.89 & 5.09\\ 
p04\_1090 & 4545.46 &  4616.62 (4656.55) & 1.56 (2.44) & 70.00 (310.84) & 4624.18 & 1.73 & 112.41 &  5214.80 & 14.72\\ 
p04\_3070 & 4334.71   & 4420.73 (4459.30) &  1.98 (2.87) & 74.35 (272.44)  & 4407.02 & 1.67 & 99.65 & 5186.12 & 19.64\\ 
p04\_7090 & 6395.41   & 6506.25 (6519.70)  &  1.73 (1.94) &  87.03 (469.62) & 6555.47  & 2.5 & 82.07  &  7360.50 & 15.09\\ 
p05\_110 &  1074.18  & 1074.58 (1103.64) &  0.04 (2.74) & 33.66 (186.66) & 1086.27 & 1.12 & 66.5 & 1089.50 & 1.42 \\ 
p05\_1030 & 2478.4   & 2500.49 (2523.97) &  0.89 (1.83) &  59.47 (241.44) & 2515.45 & 1.49 & 82.72  &  2539.43 & 2.46\\ 
p05\_1050 & 3471.41 & 3517.12 (3524.85) & 1.32 (1.54) &  75.93 (311.94) & 3510.99 & 1.14 & 87.56 & 3610.86 & 4.01\\ 
p05\_1090 & 5521.57   &  5618.96 (5632.9) &  1.76 (2.02) &  87.18 (561.54) & 5619.52 & 1.77 & 145.02&  6221.60 & 12.67\\ 
p05\_3070 & 5409.76   &  5496.88 (5540.44) & 1.61 (2.41) & 119.96 (383.28) & 5412.85 & 0.06 & 142.81 &  6252.18  & 15.57\\ 
p05\_7090 & 8192.03  & 8331.44 (8352.94)  &  1.71 (1.96) &  133.69 (884.68) & 8332.36 & 1.71 & 255.05 & 9608.41 & 17.28\\
p11\_110 & 1031.11 & 1031.11 (1052.92)  &  0.00 (2.11) & 16.19 (74.12)  &1044.44 & 1.29  & 20.20  & 1047.17 & 1.55\\ 
p11\_1030 & 2881.8   & 2881.80 (2964.84) &  0.00 (2.89) &  30.06 (94.06) &  2923.86 & 1.46  & 40.64 &  2938.20 & 1.95\\ 
p11\_1050 & 4219.01   &  4265.64 (4315.51) &  1.10 (2.29) & 39.86 (108.54)  & 4268.79  & 1.18 & 55.27  &  4333.50 & 2.71\\
p11\_1090 & 6854.09   & 7004.71 (7078.08) & 2.20 (3.27) & 64.02 (188.30)  &  6994.56 & 2.05 & 64.06 &  7760.30 & 13.22\\ 
p11\_3070 & 6671.04   &  6776.88 (6767.00) & 1.58 (1.44) &  54.73 (162.36) & 6759.99 & 1.33 & 59.01  & 7725.04 & 15.79\\ 
p11\_7090 & 10204.81  &  10364.33 (10408.39) &  1.56 (1.99) & 72.05 (231.60) & 10406.25 &  1.97 & 101.02 & 12239.31 & 19.93\\ \hline
Average &  & & 1.50 (1.96) & 45.51 (166.94) & & 1.45 & 33.38 & & 8.08 \\\hline
\end{tabular}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}[t]
\caption{Performance of RSR on Set-4}
    \centering
\begin{tabular}{ ccccccccccc }
 \hline
 Instance & Best-known &  \multicolumn{3}{c}{VRPHAS (Our runs)} &  \multicolumn{3}{c}{RSR} & \multicolumn{2}{c}{No splitting}  \\
  & & cost & gap ($\%$) & time (s) & cost & gap ($\%$) & time (s) & cost & gap ($\%$) \\
 \hline
 eil22 & 375.28 & 375.28 (375.28) & 0.00 (0.00) & 1.65 (3.28) & 375.28 & 0.00 & 3.11 & 375.28 & 0.00\\
 eil23 & 568.56 & 568.56 (568.56) & 0.00 (0.00) & 1.58 (5.92) & 568.56 & 0.00 & 2.92 & 568.56 & 0.00 \\
 eil30 & 497.53 & 497.53 (505.01) & 0.00 (1.50) & 2.18 (6.89) & 505.01 & 1.50 & 3.64 & 505.01 & 1.48 \\
 eil33 & 826.41 & 826.41 (837.67) & 0.00 (1.36) & 3.51 (6.89) & 837.67 & 1.36 & 5.08 & 837.67 & 1.36\\
 eil51 & 524.61 & 524.61 (524.61) & 0.00 (0.00) & 9.37 (12.58) & 524.61 & 0.00 & 10.95 & 524.61 & 0.00\\
 eilA76 &  823.89 & 849.60 (827.47) & 3.12 (0.43)  & 17.76 (24.60) & 830.97 & 0.86 & 19.77 & 837.45 & 1.61\\
 eilB76 & 1009.04  & 1024.44 (1028.80)  & 1.53 (1.96) & 18.81 (31.86) & 1025.24 & 1.60 & 18.65 & 1028.23 & 1.86\\
 eilC76 &  738.67 & 748.51 (742.81) &  1.33 (0.52) & 15.36 (26.78) & 742.49 & 0.55 & 17.48 & 743.48 & 0.64\\
 eilD76 & 684.53 & 684.53 (690.09) & 0.00 (0.81) & 14.72 (23.82) & 689.47 & 0.72 & 19.41  & 690.20 & 0.82\\
 eilA101 & 812.51 & 812.51 (831.65) & 0.00 (2.35) & 14.73 (55.39) & 828.98 & 2.02 & 23.37 & 827.39 & 1.92\\
 eilB101 &  1076.26  &  1099.21 (1093.13) & 2.13 (1.57) & 21.61 (30.90) & 1087.70 & 1.06 & 23.76 & 1093.02 & 1.53\\
 \hline
 Average & & & 0.74 (0.96) & 11.03 (20.80) & & 0.88 & 13.63 &  & 1.02\\
 \hline
\end{tabular}
\end{table}
\end{landscape}
